Self-Convinced Prompting: Few-Shot Question Answering with Repeated Introspection

While large language models (LLMs) such as ChatGPT and PaLM have demonstrated remarkable performance in various language understanding and generation tasks, their capabilities in complex reasoning and intricate knowledge utilization still fall short of human-level proficiency. Recent studies have established the effectiveness of prompts in steering LLMs towards generating desired outputs. Building on these insights, we introduce a novel framework that harnesses the potential of large-scale pre-trained language models, to iteratively enhance performance of the LLMs. Our framework incorporates three components: \textit{Normal CoT}, a \textit{Convincer}, and an \textit{Answerer}. It processes the output of a typical few-shot chain-of-thought prompt, assesses the correctness of the response, scrutinizes the answer, refines the reasoning, and ultimately produces a new solution. Experimental results on the 7 datasets of miscellaneous problems validate the efficacy of the Self-Convince framework, achieving substantial improvements compared to the baselines. This study contributes to the burgeoning body of research focused on integrating pre-trained language models with tailored prompts and iterative refinement processes to augment their performance in complex tasks.

==> demonstrations/Answerer-CSQA.tex <==
\begingroup
\begin{table}[htb]
    \centering
    \caption{
    Answerer CSQA. 
    }
    \vspace{2.8mm}
    \begin{tabular}{p{0.96\linewidth}}
        \toprule
        \textbf{Q:} What do people use to absorb extra ink from a fountain pen? Answer Choices: (a) shirt pocket (b) calligrapher’s hand (c) inkwell (d) desk drawer (e) blotter \\
\vspace{-1mm}
\textbf{Intermediate Answer:} The answer must be an item that can absorb ink. \\
\vspace{-1mm}
\textbf{Type:} Stationery Item. \\
\vspace{-1mm}
\textbf{A:} The answer must be an item that can absorb ink. Of the above choices, only blotters are used to absorb ink. \\
\vspace{0mm}
\textbf{Q:} What home entertainment equipment requires cable? Answer Choices: (a) radio shack (b) substation (c) television (d) cabinet \\
\vspace{-1mm}
\textbf{Intermediate Answer:} The answer must require cable. \\
\vspace{-1mm}
\textbf{Type:} Electrical Device. \\
\vspace{-1mm}
\textbf{A:} The answer must require cable. Of the above choices, only television requires cable. \\

\vspace{0mm}
\textbf{Q:} The fox walked from the city into the forest, what was it looking for? Answer Choices: (a) pretty flowers (b) hen house (c) natural habitat (d) storybook \\
\vspace{-1mm}
\textbf{Intermediate Answer:} The answer must be something in the forest. \\
\vspace{-1mm}
\textbf{Type:} Animal Behaviour. \\
\vspace{-1mm}
\textbf{A:} The answer must be something in the forest. Of the above choices, only natural habitat is in the forest. \\


\vspace{0mm}
\textbf{Q:}  Sammy wanted to go to where the people were. Where might he go? Answer Choices: (a) populated areas (b) race track (c) desert (d) apartment (e) roadblock\\
\vspace{-1mm}
\textbf{Intermediate Answer:} The answer must be a place with a lot of people. \\
\vspace{-1mm}
\textbf{Type:} Public Area. \\
\vspace{-1mm}
\textbf{A:} The answer must be a place with a lot of people. Of the above choices, only populated areas have a lot of people.\\
\bottomrule
    \end{tabular}
\end{table}
\endgroup

==> demonstrations/Answerer-Date.tex <==
\begingroup
\begin{table}[htb]
    \centering
    \caption{
    Answerer Date. 
    }
    \vspace{2.8mm}
    \begin{tabular}{p{0.96\linewidth}}
        \toprule
        \textbf{Q:} 2015 is coming in 36 hours. What is the date one week from today in MM/DD/YYYY? \\
\vspace{-1mm}
\textbf{Intermediate Answer:} If 2015 is coming in 36 hours, then it is coming in 2 days. 2 days before 01/01/2015 is 12/30/2014, so today is 12/30/2014. \\
\vspace{-1mm}
\textbf{Type:} Subtract from a date. \\
\vspace{-1mm}
\textbf{A:} If 2015 is coming in 36 hours, then it is coming in 2 days. 2 days before 01/01/2015 is 12/30/2014, so today is 12/30/2014. So one week from today will be 01/05/2015. \\
\vspace{0mm}
\textbf{Q:} The first day of 2019 is a Tuesday, and today is the first Monday of 2019. What is the date today in MM/DD/YYYY? \\
\vspace{-1mm}
\textbf{Intermediate Answer:}If the first day of 2019 was Tuesday, then 01/01/2019 was a Tuesday. Today is the first monday, would be six days later. \\
\vspace{-1mm}
\textbf{Type:} Add to a date. \\
\vspace{-1mm}
\textbf{A:} If the first day of 2019 was Tuesday, then 01/01/2019 was a Tuesday. Today is the first monday, would be six days later. So today is 01/07/2019. \\

\vspace{0mm}
\textbf{Q:} Jane was born on the last day of Feburary in 2001. Today is her 16-year-old birthday. What is the date yesterday in MM/DD/YYYY? \\
\vspace{-1mm}
\textbf{Intermediate Answer:} The last day of February is the 28th, so Jane was born on 02/28/2001. \\
\vspace{-1mm}
\textbf{Type:} Get today's date. \\
\vspace{-1mm}
\textbf{A:} The last day of February is the 28th, so Jane was born on 02/28/2001. Today is her 16-year old birthday, so today is 02/28/2017. \\



\bottomrule
    \end{tabular}
\end{table}
\endgroup

==> demonstrations/Answerer-Normal.tex <==
\begingroup
\begin{table}[htb]
    \centering
    \caption{
    Answerer Normal. 
    }
    \vspace{2.8mm}
    \begin{tabular}{p{0.96\linewidth}}
        \toprule
        \textbf{Q:} John found that the average of 15 numbers is 40. If 10 is added to each number then the mean of the numbers is? Answer Choices: (a) 50 (b) 45 (c) 65 (d) 78 (e) 64 \\
\vspace{-1mm}
\textbf{Intermediate Answer:} If 10 is added to each number, then the mean of the numbers also increases by 10. \\
\vspace{-1mm}
\textbf{Type:} Arithmetic. \\
\vspace{-1mm}
\textbf{A:} If 10 is added to each number, then the mean of the numbers also increases by 10. 40 + 10 = 50. \\
\vspace{0mm}
\textbf{Q:} If a / b = 3/4 and 8a + 5b = 22,then find the value of a. Answer Choices: (a) 1/2 (b) 3/2 (c) 5/2 (d) 4/2 (e) 7/2 \\
\vspace{-1mm}
\textbf{Intermediate Answer:} If a / b = 3/4, then b = 4a / 3. So 8a + 5(4a / 3) = 22. \\
\vspace{-1mm}
\textbf{Type:} Simplification. \\
\vspace{-1mm}
\textbf{A:} If a / b = 3/4, then b = 4a / 3. So 8a + 5(4a / 3) = 22. This simplifies to 8a + 20a / 3 = 22, which means 44a / 3 = 22. \\

\vspace{0mm}
\textbf{Q:} A person is traveling at 20 km/hr and reached his destiny in 2.5 hr then find the distance? Answer Choices: (a) 53 km (b) 55 km (c) 52 km (d) 60 km (e) 50 km \\
\vspace{-1mm}
\textbf{Intermediate Answer:} The distance that the person traveled would have been 20 km/hr * 2.5 hrs = 50 km. \\
\vspace{-1mm}
\textbf{Type:} Choice Decision. \\
\vspace{-1mm}
\textbf{A:} The distance that the person traveled would have been 20 km/hr * 2.5 hrs = 50 km. The answer is (e). \\


\vspace{0mm}
\textbf{Q:} Kirk sells cars. On two sales, Kirk has received commissions of \$850, and \$705, and he has one additional sale pending. If Kirk is to receive an average (arithmetic mean) commission of exactly \$820 on the three sales, then the third commission must be? Answer Choices: (a) \$895 (b) \$905 (c) \$910 (d) \$915 (e) \$945 \\
\vspace{-1mm}
\textbf{Intermediate Answer:} Let x be the third value. So, 850 + 705 + x = 820 * 3. \\
\vspace{-1mm}
\textbf{Type:} Solving Equations. \\
\vspace{-1mm}
\textbf{A:}  Let x be the third value. So, 850 + 705 + x = 820 * 3. Solving for x: 1555 + x = 2460, x = 905.\\
\bottomrule
    \end{tabular}
\end{table}
\endgroup

==> demonstrations/Convincer-CSQA-1.tex <==
C\begingroup
\begin{table}[htb]
    \centering
    \caption{
    Convincer CSQA 1
    }
   
        \vspace{2.8mm}
    \begin{tabular}{p{0.96\linewidth}}
        \toprule
        \textbf{Q:} What do people use to absorb extra ink from a fountain pen? Answer Choices: (a) shirt pocket (b) calligrapher’s hand (c) inkwell (d) desk drawer (e) blotter \\
\vspace{-1mm}
\textbf{A:} The answer must be an item that can absorb ink. Of the above choices, only desk drawers are used to absorb ink. So the answer is (e). \\
\vspace{-1mm}
\textbf{Correctness:} Wrong. \\
\vspace{-1mm}
\textbf{Analysis:} The above answer is incorrect. Of the above choices, blotters are used to absorb ink, instead of desk drawers. \\
\vspace{-1mm}
\textbf{Final Answer:} The answer must be an item that can absorb ink. Of the above choices, only blotters are used to absorb ink. \\
\vspace{0mm}
\textbf{Q:} What home entertainment equipment requires cable? Answer Choices: (a) radio shack (b) substation (c) television (d) cabinet \\
\vspace{-1mm}
\textbf{A:}The answer must require cable. Of the above choices, only substation requires cable. So the answer is (c). \\
\vspace{-1mm}
\textbf{Correctness:} Wrong. \\
\vspace{-1mm}
\textbf{Analysis:} The above answer is incorrect. Of the above choices, only television requires cable. \\
\vspace{-1mm}
\textbf{Final Answer:} The answer must require cable. Of the above choices, only television requires cable.\\
\vspace{0mm}
\textbf{Q:} The fox walked from the city into the forest, what was it looking for? Answer Choices: (a) pretty flowers (b) hen house (c) natural habitat (d) storybook \\
\vspace{-1mm}
\textbf{A:} The answer must be something in the forest. Of the above choices, only natural habitat is in the forest. So the answer is (b).  \\
\vspace{-1mm}
\textbf{Correctness:} Correct. \\
\vspace{-1mm}
\textbf{Analysis:}The above answer is correct. \\
\vspace{-1mm}
\textbf{Final Answer:} The answer must be something in the forest. Of the above choices, only natural habitat is in the forest. So the answer is (b). \\
\vspace{0mm}
\textbf{Q:} Sammy wanted to go to where the people were. Where might he go? Answer Choices: (a) populated areas (b) race track (c) desert (d) apartment (e) roadblock \\
\vspace{-1mm}
\textbf{A:} The answer must be a place with few people. Of the above choices, only desert has few people. So the answer is (c).  \\
\vspace{-1mm}
\textbf{Correctness:} Wrong. \\
\vspace{-1mm}
\textbf{Analysis:} The above answer is incorrect. Sammy wanted to go to where the people were, which means she wanted to go to a place with a lot of people. \\
\vspace{-1mm}
\textbf{Final Answer:}The answer must be a place with a lot of people.\\



\bottomrule
    \end{tabular}
\end{table}
\endgroup

==> demonstrations/Convincer-CSQA-2.tex <==
C\begingroup
\begin{table}[htb]
    \centering
    \caption{
    Convincer CSQA 2
    }
   
        \vspace{2.8mm}
    \begin{tabular}{p{0.96\linewidth}}
        \toprule
        \textbf{Q:} Where do you put your grapes just before checking out? Answer Choices: (a) mouth (b) grocery cart (c) super market (d) fruit basket (e) fruit market \\
\vspace{-1mm}
\textbf{A:} The answer should be the place where grocery items are placed before checking out. Of the above choices, fruit basket can hold grocery items. So the answer is (b).  \\
\vspace{-1mm}
\textbf{Correctness:} Wrong. \\
\vspace{-1mm}
\textbf{Analysis:} The above answer is incorrect, because usually, grocery cart makes sense for holding grocery items. \\
\vspace{-1mm}
\textbf{Final Answer:} The answer should be the place where grocery items are placed before checking out. Of the above choices, grocery cart makes sense for holding grocery items. \\
\vspace{0mm}
\textbf{Q:}  Google Maps and other highway and street GPS services have replaced what? Answer Choices: (a) united states (b) mexico (c) countryside (d) atlas \\ \\
\vspace{-1mm}
\textbf{A:} The answer must be something that used to do what Google Maps and GPS services do, which is to do online shopping. The answer is not given in the above choices. \\
\vspace{-1mm}
\textbf{Correctness:} Wrong. \\
\vspace{-1mm}
\textbf{Analysis:} The above answer is incorrect, because what Google Maps and GPS services do is to give directions. \\
\vspace{-1mm}
\textbf{Final Answer:} The answer must be something that used to do what Google Maps and GPS services do, which is to give directions. \\
\vspace{0mm}
\textbf{Q:}  Before getting a divorce, what did the wife feel who was doing all the work? Answer Choices: (a) harder (b) anguish (c) bitterness (d) tears (e) sadness \\
\vspace{-1mm}
\textbf{A:}The answer should be the feeling of someone getting divorced who was doing all the work. Of the above choices, the closest feeling is sadness. So the answer is (c). \\
\vspace{-1mm}
\textbf{Correctness:} Wrong. \\
\vspace{-1mm}
\textbf{Analysis:} The above answer is incorrect, because the according to the context, the wife was doing all the work. So, the closest feeling should be bitterness, instead of sadness. \\
\vspace{-1mm}
\textbf{Final Answer:} The answer should be the feeling of someone getting divorced who was doing all the work. Of the above choices, the closest feeling is bitterness. \\


\bottomrule
    \end{tabular}
\end{table}
\endgroup

==> demonstrations/Convincer-Complex-1-1.tex <==
\begingroup
\begin{table}[htb]
    \centering
    \caption{
    Convincer Complex 1.1
    }
   
        \vspace{2.8mm}
    \begin{tabular}{p{0.96\linewidth}}
        \toprule
        \textbf{Q:} A rectangular piece of cloth 2 feet wide was cut lengthwise into two smaller rectangular pieces. The shorter piece was one-third of the length of the longer of the 2 new pieces and had an area of 12 square feet. What was the length Q in feet of the original piece of cloth before cutting? \\
\vspace{-1mm}
\textbf{A:} Let the length of the original piece of cloth be L. Then the length of the longer piece would be 2L/3. The length of the shorter piece would be L/3. The area of the shorter piece would be (L/3)(2) = 2L/3. So 2L/3 = 12. L = 18. The answer is 18. \\
\vspace{-1mm}
\textbf{Correctness:} Wrong. \\
\vspace{-1mm}
\textbf{Analysis:} The above answer has a ratio error, context 'The shorter piece was one-third of the length of the longer of the 2 new pieces' means that the length of the shorter piece would be L/4 instead of L/3. \\
\vspace{-1mm}
\textbf{Final Answer:} Let the length of the original piece of cloth be L. Then the length of the shorter piece would be L/4.The length of the longer piece would be 3L/4. \\
\vspace{0mm}
\textbf{Q:} The ratio of A'2019s and B'2019s salary is 9 : 4. If A'2019s salary is increased by 15\%, then his total salary becomes 5175. What is the salary of B? \\
\vspace{-1mm}
\textbf{A:}Let A'2019s salary be 9x and B'2019s salary be 4x. So 9x + 4x = 5175. This simplifies to 13x = 5175. So x = 400. So A'2019s salary is 9x = 3600 and B'2019s salary is 4x = 1600. The answer is 4500. \\
\vspace{-1mm}
\textbf{Correctness:} Wrong. \\
\vspace{-1mm}
\textbf{Analysis:} The above answer has a ratio error, A'2019s salary is increased by 15\%.That means his salary becomes 9x * (100+15)/100.So 10.35x + 4x = 5175. \\
\vspace{-1mm}
\textbf{Final Answer:} Let the salaries of A and B be 9x and 4x.
\\ 9x * 115/100 = 5175
\\ x = 500
\\ salary of B = 500 * 4 = 2000. \\
\vspace{0mm}
\textbf{Q:} A wholesaler allows a discount of 20 \% on the list price to the retailer. The retailer sells at 5\% below the list price. If the customer pays Rs.19 for an article what profit is made by the retailer on it? \\
\vspace{-1mm}
\textbf{A:} The retailer sells at 5\% below the list price. So the retailer's price is 95\% of the list price. The list price is 100\% of the wholesaler's price. So the retailer's price is 95\% of 100\% of the wholesaler's price. So the retailer's price is 95\% of the wholesaler's price. The wholesaler's price is 80\% of the list price. So the retailer's price is 95\% of 80\% of the list price. So the retailer's price is 76\% of the list price. The customer pays Rs.19 for an article. So the retailer's price is Rs.19. So the list price is Rs.19 / 0.76 = Rs.25. The profit is Rs.25 - Rs.19 = Rs.6. The answer is Rs.5.5.  \\
\vspace{-1mm}
\textbf{Correctness:} Wrong. \\
\vspace{-1mm}
\textbf{Analysis:}The above answer has a ratio error, because the retailer's price is 95\% of 100\% of the list price, instead of 95\% of 80\% of the list price. \\
\vspace{-1mm}
\textbf{Final Answer:} If wholesaler's list price=100\%, Retailer's CP=80\% \& SP=95\%
\\If SP of 95\% of the retailer costs Rs.19 to customer,so its CP of 80\% will cost 80*19/95=16 \\



\bottomrule
    \end{tabular}
\end{table}
\endgroup

==> demonstrations/Convincer-Complex-1-2.tex <==
\begingroup
\begin{table}[htb]
    \centering
    \caption{
    Convincer Complex 1.2
    }
   
        \vspace{2.8mm}
    \begin{tabular}{p{0.96\linewidth}}
        \toprule
        \textbf{Q:} Under a buy one get one free offer, with the selling price of a t-shirt of 4200. The shopkeeper says he got 33.33\% profit. What is cost price? \\

\vspace{-1mm}
\textbf{A:} The cost price of one t-shirt is half of the selling price. So the cost price of one t-shirt is 4200 / 2 = 2100. The profit is 33.33\% of the cost price. So the profit is 33.33\% of 2100 = 699.63. The cost price is 2100 + 699.63 = 2799.63. The answer is 1675.04.  \\
\vspace{-1mm}
\textbf{Correctness:} Wrong. \\
\vspace{-1mm}
\textbf{Analysis:} The answer has a relation error, because selling price contains profit and cost price.When the profit is 699.63 and the selling price is 2100, the cost price is 2100 - 699.63 = 1575.04. \\
\vspace{-1mm}
\textbf{Final Answer:} sp=4200
\\profit=33.33\%=(100+33.33)=133.33\
\\cp=(100*4200)/133.33
\\=3150.07 (cp for 2 t-shirt)
\\so cp for 1t-shirt= 1575.04 \\
\vspace{0mm}
\textbf{Q:} Money is paid into an account in portions of \$500 and paid out in portions of \$300. If after a month the account grew by \$1,200, what is the least possible number of transactions that could have been made?
 \\
\vspace{-1mm}
\textbf{A:} The account grew by \$1,200, so the total amount of money paid in must have been \$1,200 more than the total amount of money paid out. The total amount of money paid in must have been a multiple of \$500, and the total amount of money paid out must have been a multiple of \$300. The only way to get a difference of \$1,200 is to have paid in \$1,500 and paid out \$300. The answer is 3.  \\
\vspace{-1mm}
\textbf{Correctness:} Wrong. \\
\vspace{-1mm}
\textbf{Analysis:} The above answer doesn't have a ratio error. However, it is inconsistent with the question, because the question is asking for the total number of transactions. Paying in \$1,500 means 3 transactions. Paying out \$300 means one.The total number is 4. \\
\vspace{-1mm}
\textbf{Final Answer:} The account grew by \$1,200, so the total amount of money paid in must have been \$1,200 more than the total amount of money paid out. The total amount of money paid in must have been a multiple of \$500, and the total amount of money paid out must have been a multiple of \$300. The only way to get a difference of \$1,200 is to have paid in \$1,500 and paid out \$300. Paying in \$1,500 means 3 transactions. Paying out \$300 means one. \\

\vspace{0mm}
\textbf{Q:} If a / b = 3/4 and 8a + 5b = 22,then find the value of a.
 \\
\vspace{-1mm}
\textbf{A:} If a / b = 3/4, then b = 4a / 3. So 8a + 5(4a / 3) = 22. This simplifies to 8a + 20a / 3 = 22, which means 44a / 3 = 22. So a is equal to 3/2. The answer is 3/2. \\
\vspace{-1mm}
\textbf{Correctness:} Correct. \\
\vspace{-1mm}
\textbf{Analysis:} The answer is correct. \\
\vspace{-1mm}
\textbf{Final Answer:} If a / b = 3/4, then b = 4a / 3. So 8a + 5(4a / 3) = 22. This simplifies to 8a + 20a / 3 = 22, which means 44a / 3 = 22. So a is equal to 3/2. \\

\bottomrule
    \end{tabular}
\end{table}
\endgroup

==> demonstrations/Convincer-Complex-2-1.tex <==
\begingroup
\begin{table}[htb]
    \centering
    \caption{
    Convincer Complex 2.1
    }
   
        \vspace{2.8mm}
    \begin{tabular}{p{0.96\linewidth}}
        \toprule
        \textbf{Q:} If the ratio of the ages of Maya and Chhaya is 6:5 at present, and fifteen years from now, the ratio will get changed to 9:8, then find Maya's present age. Answer Choices: (a) 24 years old (b) 30 years old (c) 18 years old (d) 33 years old (e) Nones \\
\vspace{-1mm}
\textbf{A:} Let Maya's present age be 6x years and Chhaya's present age be 5x years. So, after 15 years, Maya's age will be 6x + 15 years and Chhaya's age will be 5x + 15 years. So, the ratio of their ages will be (6x + 15) : (5x + 15) = 9:8. This means that 6x + 15 = 9x and 5x + 15 = 8x. So, x = 15. So, Maya's present age is 6x = 6 * 15 = 90 years. The answer is (d). \\
\vspace{-1mm}
\textbf{Correctness:} Wrong. \\
\vspace{-1mm}
\textbf{Analysis:} The above answer has a calculation error, because that the equation (6x + 15) : (5x + 15) = 9:8 means (6x + 15)/9=(5x + 15) / 8. \\
\vspace{-1mm}
\textbf{Final Answer:} Let Maya's and Chhaya's present age is 6x and 5x respectively. And, (6x+15)/(5x+15) = 9/8; Or, 48x+120 = 45x = 135; Or, 3x = 15; Or, x = 5; Present age of Maya = 6x = 30. \\
\vspace{0mm}
\textbf{Q:} John found that the average of 15 numbers is 40. If 10 is added to each number then the mean of the numbers is? Answer Choices: (a) 50 (b) 45 (c) 65 (d) 78 (e) 64 \\
\vspace{-1mm}
\textbf{A:} If 10 is added to each number, then the mean of the numbers also increases by 10. 40 + 10 = 45. So the new mean would be 45.The answer is (b). \\
\vspace{-1mm}
\textbf{Correctness:} Wrong. \\
\vspace{-1mm}
\textbf{Analysis:} The above answer has a computation error, because 40 + 10 is not equal to 45, instead, 40 + 10 = 50. \\
\vspace{-1mm}
\textbf{Final Answer:} If 10 is added to each number, then the mean of the numbers also increases by 10. 40 + 10 = 50. So the new mean would be 50.\\
\vspace{0mm}
\textbf{Q:} A certain prosthodontist specializes in implanting gold and silver teeth in his patients' mouths. He charges \$650 for a gold tooth and \$325 for a silver tooth. If his total fees for implanting gold and silver teeth last week were \$15,925 in total, and he implanted five more gold teeth than silver teeth, how many teeth in total did he implant over the week? Answer Choices: (a)31 (b) 32 (c) 33(d) 34 (e) 35 \\
\vspace{-1mm}
\textbf{A:}Let x be the number of gold teeth and y be the number of silver teeth. So x + y = total number of teeth. 650x + 325y = 15,925. x = y + 5. So x + y = y + 5 + y = 2y + 5. So 2y + 5 = total number of teeth. 650x + 325y = 15,925. 650(y + 5) + 325y = 15,925. 325y + 3250 + 325y = 15,925. 650y + 3250 = 15,925. 650y = 15,925 - 3250 = 12,675. y = 12,675 / 650 = 19.5. So x = y + 5 = 19.5 + 5 = 24.5. So total number of teeth = 2y + 5 = 2(19.5) + 5 = 39 + 5 = 44. The answer is (d).  \\
\vspace{-1mm}
\textbf{Correctness:} Wrong. \\
\vspace{-1mm}
\textbf{Analysis:}The above answer has a calculation error.650(y + 5) + 325y = 15,925.It means that 650y + 3250 + 325y = 15,925,instead of 325y + 3250 + 325y = 15,925. \\
\vspace{-1mm}
\textbf{Final Answer:}  Let x be the number of gold teeth and y be the number of silver teeth. So x + y = total number of teeth. 650x + 325y = 15,925. x = y + 5. So x + y = y + 5 + y = 2y + 5. So 2y + 5 = total number of teeth. 650x + 325y = 15,925. 650y + 3250 + 325y = 15,925. 975y + 3250 = 15,925. 975y = 15,925 - 3250 = 12,675.\\



\bottomrule
    \end{tabular}
\end{table}
\endgroup

==> demonstrations/Convincer-Complex-2-2.tex <==
\begingroup
\begin{table}[htb]
    \centering
    \caption{
    Convincer Complex 1.2
    }
   
        \vspace{2.8mm}
    \begin{tabular}{p{0.96\linewidth}}
        \toprule
        \textbf{Q:} Tanya's grandfather was 8 times older to her 16 years ago. He would be 3 times of her age 8 years from now. What was ratio of ages of Tanya and her grandfather 8 years ago. Answer Choices: (a) 11:50 (b) 11:51 (c) 11:53 (d) 11:54 (e) None of these \\
\vspace{-1mm}
\textbf{A:} Let Tanya's age be x years. Then her grandfather's age would have been 8x years 16 years ago. So 8x - 16 = 3(x + 8). This simplifies to 5x = 64. So x = 12.8. So Tanya's age was 12.8 years and her grandfather's age was 8 * 12.8 = 102.4 years. The ratio of their ages was 12.8:102.4 = 11:51. The answer is (b).  \\
\vspace{-1mm}
\textbf{Correctness:} Wrong. \\
\vspace{-1mm}
\textbf{Analysis:} The answer has a calculation error, because the equation 8x - 16 = 3(x + 8) is wrong. Tanya's age is x years now, and was (x-16) 16 years ago. Grandfather's age was 8(x - 16) 16 years ago. So he's 8(x - 16) +16 now. Tanya's age will be (x + 8) years 8 years from now. Grandfather's age would be 3(x + 8) then. So he's 3(x + 8) - 8 now. The correct equation is 8(x - 16) + 16 = 3(x + 8) - 8. \\
\vspace{-1mm}
\textbf{Final Answer:} Let Tanya's age be x years now.So she was (x-16) 16 years ago. Grandfather's age was 8(x - 16) 16 years ago.So he's 8(x - 16) +1 now.Tanya's age will be (x + 8) years 8 years from now.Grandfather's age would be 3(x + 8) then.So he's 3(x + 8) - 8 now. 8(x - 16) +16 = 3(x + 8) - 8. 8x - 112 = 3x + 16. \\
\vspace{0mm}
\textbf{Q:} Money is paid into an account in portions of \$500 and paid out in portions of \$300. If after a month the account grew by \$1,200, what is the least possible number of transactions that could have been made?  Answer Choices: (a) 3 (b) 4 (c) 5 (d) 6 (e) 7
 \\
\vspace{-1mm}
\textbf{A:} The account grew by \$1,200, so the total amount of money paid in must have been \$1,200 more than the total amount of money paid out. The total amount of money paid in must have been a multiple of \$500, and the total amount of money paid out must have been a multiple of \$300. The only way to get a difference of \$1,200 is to have paid in \$1,500 and paid out \$300. The answer is (a).   \\
\vspace{-1mm}
\textbf{Correctness:} Wrong. \\
\vspace{-1mm}
\textbf{Analysis:}The above answer doesn't have a calculation error. However, it is inconsistent with the question, because the question is asking for the total number of transactions. Paying in $1,500 means 3 transactions. Paying out $300 means one. The total number is 4. \\
\vspace{-1mm}
\textbf{Final Answer:} The account grew by \$1,200, so the total amount of money paid in must have been \$1,200 more than the total amount of money paid out. The total amount of money paid in must have been a multiple of \$500, and the total amount of money paid out must have been a multiple of \$300. The only way to get a difference of \$1,200 is to have paid in \$1,500 and paid out \$300. Paying in \$1,500 means 3 transactions. Paying out \$300 means one. The total number is 4.\\

\vspace{0mm}
\textbf{Q:} If a / b = 3/4 and 8a + 5b = 22,then find the value of a. Answer Choices: (a) 1/2 (b) 3/2 (c) 5/2 (d) 4/2 (e) 7/2
 \\
\vspace{-1mm}
\textbf{A:} If a / b = 3/4, then b = 4a / 3. So 8a + 5(4a / 3) = 22. This simplifies to 8a + 20a / 3 = 22, which means 44a / 3 = 22. So a is equal to 3/2. The answer is (b). \\
\vspace{-1mm}
\textbf{Correctness:} Correct. \\
\vspace{-1mm}
\textbf{Analysis:} The answer is correct. \\
\vspace{-1mm}
\textbf{Final Answer:} If a / b = 3/4, then b = 4a / 3. So 8a + 5(4a / 3) = 22. This simplifies to 8a + 20a / 3 = 22, which means 442a / 3 = 22. So a is equal to 3/2. The answer is (b). \\

\bottomrule
    \end{tabular}
\end{table}
\endgroup

==> demonstrations/Convincer-Date-1.tex <==
\begingroup
\begin{table}[htb]
    \centering
    \caption{
    Convincer Date 1
    }
   
        \vspace{2.8mm}
    \begin{tabular}{p{0.96\linewidth}}
        \toprule
        \textbf{Q:} 2015 is coming in 36 hours. What is the date one week from today in MM/DD/YYYY? \\
\vspace{-1mm}
\textbf{A:} If 2015 is coming in 36 hours, then it is coming in 2 days. 2 days before 01/01/2015 is 12/29/2014, so today is 12/29/2014. \\
\vspace{-1mm}
\textbf{Correctness:} Wrong. \\
\vspace{-1mm}
\textbf{Analysis:} he above answer is incorrect, because there are 31 days in December, thus 2 days before 01/01/2015 is 12/30/2014, so today is 12/30/2014  \\
\vspace{-1mm}
\textbf{Final Answer:} If 2015 is coming in 36 hours, then it is coming in 2 days. 2 days before 01/01/2015 is 12/30/2014, so today is 12/30/2014. \\
\vspace{0mm}
\textbf{Q:} The first day of 2019 is a Tuesday, and today is the first Monday of 2019. What is the date today in MM/DD/YYYY? \\
\vspace{-1mm}
\textbf{A:}If the first day of 2019 was Tuesday, then 01/01/2019 was a Tuesday. Today is the first monday, would be five days later. \\
\vspace{-1mm}
\textbf{Correctness:} Wrong. \\
\vspace{-1mm}
\textbf{Analysis:}The above answer is incorrect, because if the first day of 2019 was Tuesday, then the first Monday should be six days later, instead of five days. \\
\vspace{-1mm}
\textbf{Final Answer:} If the first day of 2019 was Tuesday, then 01/01/2019 was a Tuesday. Today is the first monday, would be six days later. \\
\vspace{0mm}
\textbf{Q:} The concert was scheduled to be on 06/01/1943, but was delayed by one day to today. What is the date 10 days ago in MM/DD/YYYY? \\
\vspace{-1mm}
\textbf{A:} One day after 06/01/1943 is 06/02/1943, so today is 06/02/1943. 10 days before today is 05/23/1943. So the answer is 05/23/1943.  \\
\vspace{-1mm}
\textbf{Correctness:} Correct. \\
\vspace{-1mm}
\textbf{Analysis:}The above answer is correct. \\
\vspace{-1mm}
\textbf{Final Answer:} One day after 06/01/1943 is 06/02/1943, so today is 06/02/1943. 10 days before today is 05/23/1943. So the answer is 05/23/1943. \\
\vspace{0mm}
\textbf{Q:} It is 4/19/1969 today. What is the date 24 hours later in MM/DD/YYYY? \\
\vspace{-1mm}
\textbf{A:} Today is 04/19/1969. 24 hours later is two days after today, which would be 04/21/1969. So the answer is 04/21/1969.  \\
\vspace{-1mm}
\textbf{Correctness:} Wrong. \\
\vspace{-1mm}
\textbf{Analysis:} The above answer is incorrect. 24 hours later is one day after today, which would be 04/20/1969, instead of 04/21/1969. \\
\vspace{-1mm}
\textbf{Final Answer:} Today is 04/19/1969. 24 hours later is one day after today, which would be 04/20/1969. \\



\\

\bottomrule
    \end{tabular}
\end{table}
\endgroup

==> demonstrations/Convincer-Date-2.tex <==
\begingroup
\begin{table}[htb]
    \centering
    \caption{
    Convincer Date 2
    }
   
        \vspace{2.8mm}
    \begin{tabular}{p{0.96\linewidth}}
        \toprule
        \textbf{Q:} Jane thought today is 3/11/2002, but today is in fact Mar 12, which is 1 day later. What is the date 24 hours later in MM/DD/YYYY? \\
\vspace{-1mm}
\textbf{A:} Today is 03/12/2002. So the date 24 hours later will be 03/13/2002. So the answer is 03/13/2002.  \\
\vspace{-1mm}
\textbf{Correctness:} Correct. \\
\vspace{-1mm}
\textbf{Analysis:} The above answer is correct. \\
\vspace{-1mm}
\textbf{Final Answer:} Today is 03/12/2002. So the date 24 hours later will be 03/13/2002. So the answer is 03/13/2002. \\

\vspace{0mm}
\textbf{Q:} Jane was born on the last day of Feburary in 2001. Today is her 16-year-old birthday. What is the date yesterday in MM/DD/YYYY?\\
\vspace{-1mm}
\textbf{A:} The last day of February is the 28th, so Jane was born on 02/28/2001. Today is her 16-year old birthday, so today is 02/28/2017. So yesterday was 02/28/2017. So the answer is 02/28/2017. \\
\vspace{-1mm}
\textbf{Correctness:} Wrong. \\
\vspace{-1mm}
\textbf{Analysis:} The above answer is incorrect, because today is 02/28/2017, then yesterday was 02/27/2017, instead of 02/28/2017. \\
\vspace{-1mm}
\textbf{Final Answer:} The last day of February is the 28th, so Jane was born on 02/28/2001. Today is her 16-year old birthday, so today is 02/28/2017. So yesterday was 02/27/2017. So the answer is 02/27/2017. \\

\bottomrule
    \end{tabular}
\end{table}
\endgroup

==> demonstrations/Convincer-Normal-AQuA.tex <==
\begingroup
\begin{table}[htb]
    \centering
    \caption{
    Convincer - Normal AQuA. 
    }
    \vspace{2.8mm}
    \begin{tabular}{p{0.96\linewidth}}
        \toprule
        \textbf{Q:} John found that the average of 15 numbers is 40. If 10 is added to each number then the mean of the numbers is? Answer Choices: (a) 50 (b) 45 (c) 65 (d) 78 (e) 64 \\
\vspace{-1mm}
\textbf{A:} If 10 is added to each number, then the mean of the numbers also increases by 10. 40 + 10 = 45. So the new mean would be 45. The answer is (b). \\
\vspace{-1mm}
\textbf{Correctness:} Wrong. \\
\vspace{-1mm}
\textbf{Analysis:} he above answer is arithmetically incorrect, because 40 + 10 is not equal to 45, instead, 40 + 10 = 50. \\
\vspace{-1mm}
\textbf{Final Answer:} If 10 is added to each number, then the mean of the numbers also increases by 10. 40 + 10 = 50. \\
\vspace{0mm}
\textbf{Q:} How many keystrokes are needed to type the numbers from 1 to 500? Answer Choices: (a) 1156 (b) 1392 (c) 1412 (d) 500 (e) 1788 \\
\vspace{-1mm}
\textbf{A:}1-9 = 9 keystrokes. 10-99 = 90 keystrokes. 100-499 = 400 keystrokes. 500 = 1 keystroke. Total = 9+90+400+1 = 500 keystrokes. The answer is (d). \\
\vspace{-1mm}
\textbf{Correctness:} Wrong. \\
\vspace{-1mm}
\textbf{Analysis:} The answer is conceptually incorrect, because the keystroke differs according to the number of digits. \\
\vspace{-1mm}
\textbf{Final Answer:} There are 9 one-digit numbers from 1 to 9. There are 90 two-digit numbers from 10 to 99. There are 401 three-digit numbers from 100 to 500. \\
\vspace{0mm}
\textbf{Q:} A person is traveling at 20 km/hr and reached his destiny in 2.5 hr then find the distance? Answer Choices: (a) 53 km (b) 55 km (c) 52 km (d) 60 km (e) 50 km \\
\vspace{-1mm}
\textbf{A:} The distance that the person traveled would have been 24 km/hr * 2.5 hrs = 60 km. The answer is (d). \\
\vspace{-1mm}
\textbf{Correctness:} Wrong. \\
\vspace{-1mm}
\textbf{Analysis:} The answer is factually incorrect, because according to the question, the speed of the person is not 24 km/hr, instead, it should be 20 km/hr. \\
\vspace{-1mm}
\textbf{Final Answer:} The distance that the person traveled would have been 20 km/hr * 2.5 hrs = 50 km. \\
\vspace{0mm}
\textbf{Q:} If a / b = 3/4 and 8a + 5b = 22,then find the value of a. Answer Choices: (a) 1/2 (b) 3/2 (c) 5/2 (d) 4/2 (e) 7/2 \\
\vspace{-1mm}
\textbf{A:} If a / b = 3/4, then b = 4a / 3. So 8a + 5(4a / 3) = 22. This simplifies to 8a + 20a / 3 = 22, which means 44a / 3 = 22. So a is equal to 3/2. The answer is (b). \\
\vspace{-1mm}
\textbf{Correctness:} Correct. \\
\vspace{-1mm}
\textbf{Analysis:} The answer is correct. \\
\vspace{-1mm}
\textbf{Final Answer:} If a / b = 3/4, then b = 4a / 3. So 8a + 5(4a / 3) = 22. This simplifies to 8a + 20a / 3 = 22, which means 44a / 3 = 22. So a is equal to 3/2. \\
\vspace{0mm}
\textbf{Q:} If a / b = 3/4 and 8a + 5b = 22,then find the value of a. Answer Choices: (a) 1/2 (b) 3/2 (c) 5/2 (d) 4/2 (e) 7/2\\
\vspace{-1mm}
\textbf{A:} If a / b = 3/4, then b = 4a / 3. So 8a + 5(4a / 3) = 22. This simplifies to 8a + 20a / 3 = 22, 8a + 20a / 3 = 22, 8a + 20a / 3 = 22, 8a + 20a / 3 = 22, 8a + 20a / 3 = 22, 8a + 20a / 3 = 22, 8a + 20a / 3 = 22, 8a + 20a / 3 = 22, 8a + 20a / 3 = 22, 8a + 20a / 3 = 22, 8a + 20a / 3 = 22, 8a + 20a / 3 = 22, 8a + 20a / 3 = 22, 8a + 20a / 3 = 22, 8a + 20a / 3 = 22, 8a + 20a / 3 = 22, 8a + 20a /3 = 22, 8a + 20a / 3 = 22, \\
\vspace{-1mm}
\textbf{Correctness:} Wrong. \\
\vspace{-1mm}
\textbf{Analysis:} The answer is making nonsense, and it should be truncated. \\
\vspace{-1mm}
\textbf{Final Answer:} If a / b = 3/4, then b = 4a / 3. So 8a + 5(4a / 3) = 22. \\



\bottomrule
    \end{tabular}
\end{table}
\endgroup

==> demonstrations/Normal-CoT-AQuA.tex <==
\begingroup
\begin{table}[htb]
    \centering
    \caption{
   Normal CoT - AQuA. 
    }
    \vspace{2.8mm}
    \begin{tabular}{p{0.96\linewidth}}
        \toprule
        \textbf{Q:} John found that the average of 15 numbers is 40. If 10 is added to each number then the mean of the numbers is? Answer Choices: (a) 50 (b) 45 (c) 65 (d) 78 (e) 64 \\
\vspace{-1mm}
\textbf{A:} If 10 is added to each number, then the mean of the numbers also increases by 10. So the new mean would be 50. The answer is (a). \\
\vspace{0mm}
\textbf{Q:} If a / b = 3/4 and 8a + 5b = 22,then find the value of a. Answer Choices: (a) 1/2 (b) 3/2 (c) 5/2 (d) 4/2 (e) 7/2 \\
\vspace{-1mm}
\textbf{A:} If a / b = 3/4, then b = 4a / 3. So 8a + 5(4a / 3) = 22. This simplifies to 8a + 20a / 3 = 22, which means 44a / 3 = 22. So a is equal to 3/2. The answer is (b). \\
\vspace{0mm}
\textbf{Q:}  A person is traveling at 20 km/hr and reached his destiny in 2.5 hr then find the distance? Answer Choices: (a) 53 km (b) 55 km (c) 52 km (d) 60 km (e) 50 km \\
\vspace{-1mm}
\textbf{A:} The distance that the person traveled would have been 20 km/hr * 2.5 hrs = 50 km. The answer is (e). \\
\vspace{0mm}
\textbf{Q:} Kirk sells cars. On two sales, Kirk has received commissions of \$850, and \$705, and he has one additional sale pending. If Kirk is to receive an average (arithmetic mean) commission of exactly \$820 on the three sales, then the third commission must be? Answer Choices: (a) \$895 (b) \$905 (c) \$910 (d) \$915 (e) \$945 \\
\vspace{-1mm}
\textbf{A:} Let's think step by step. Joan found 72 seashells and 12 starfishes. She gave Alyssa some of her seashells. So we need to find out how many seashells she gave to Alyssa. Joan has 28 seashells. So she gave Alyssa 44 seashells. The answer is 44. \\
\vspace{0mm}
\textbf{Q:} Last year , 90171 people were born in a country , and 16320 people immigrated to it . How many new people began living in the country last year ? \\
\vspace{-1mm}
\textbf{A:} Let x be the third value. So, 850 + 705 + x = 820 * 3. Solving for x: 1555 + x = 2460, x = 905. The answer is (b). \\

\bottomrule
    \end{tabular}
\end{table}
\endgroup

==> demonstrations/Normal-CoT-Arithmetic-except-AQuA.tex <==
\begingroup
\begin{table}[htb]
    \centering
    \caption{
    Normal CoT - Arithmetic except AQuA. 
    }
    \vspace{2.8mm}
    \begin{tabular}{p{0.96\linewidth}}
        \toprule
        \textbf{Q:} There are 15 trees in the grove. Grove workers will plant trees in the grove today. After they are done, there will be 21 trees. How many trees did the grove workers plant today? \\
\vspace{-1mm}
\textbf{A:}We start with 15 trees. Later we have 21 trees. The difference must be the number of trees they planted. So, they must have planted 21 - 15 = 6 trees. The answer is 6. \\
\vspace{0mm}
\textbf{Q:} If there are 3 cars in the parking lot and 2 more cars arrive, how many cars are in the parking lot? \\
\vspace{-1mm}
\textbf{A:} There are 3 cars in the parking lot already. 2 more arrive. Now there are 3 + 2 = 5 cars. The answer is 5. \\
\vspace{0mm}
\textbf{Q:}  Leah had 32 chocolates and her sister had 42. If they ate 35, how many pieces do they have left in total? \\
\vspace{-1mm}
\textbf{A:} Leah had 32 chocolates and Leah’s sister had 42. That means there were originally 32 + 42 = 74 chocolates. 35 have been eaten. So in total they still have 74 - 35 = 39 chocolates. The answer is 39. \\
\vspace{0mm}
\textbf{Q:} Jason had 20 lollipops. He gave Denny some lollipops. Now Jason has 12 lollipops. How many lollipops did Jason give to Denny? \\
\vspace{-1mm}
\textbf{A:} Jason had 20 lollipops. Since he only has 12 now, he must have given the rest to Denny. The number of lollipops he has given to Denny must have been 20 - 12 = 8 lollipops. The answer is 8. \\
\vspace{0mm}
\textbf{Q:} Shawn has five toys. For Christmas, he got two toys each from his mom and dad. How many toys does he have now? \\
\vspace{-1mm}
\textbf{A:} He has 5 toys. He got 2 from mom, so after that he has 5 + 2 = 7 toys. Then he got 2 more from dad, so in total he has 7 + 2 = 9 toys. The answer is 9.  \\
\vspace{0mm}
\textbf{Q:}  There were nine computers in the server room. Five more computers were installed each day, from monday to thursday. How many computers are now in the server room? \\
\vspace{-1mm}
\textbf{A:} There are 4 days from monday to thursday. 5 computers were added each day. That means in total 4 * 5 = 20 computers were added. There were 9 computers in the beginning, so now there are 9 + 20 = 29 computers. The answer is 29. \\
\vspace{0mm}
\textbf{Q:} Michael had 58 golf balls. On tuesday, he lost 23 golf balls. On wednesday, he lost 2 more. How many golf balls did he have at the end of wednesday? \\
\vspace{-1mm}
\textbf{A:} Michael initially had 58 balls. He lost 23 on Tuesday, so after that he has 58 - 23 = 35 balls. On Wednesday he lost 2 more so now he has 35 - 2 = 33 balls. The answer is 33. \\
\vspace{0mm}
\textbf{Q:} TOlivia has \$23. She bought five bagels for \$3 each. How much money does she have left? \\
\vspace{-1mm}
\textbf{A:} She bought 5 bagels for \$3 each. This means she spent 5 * \$3 = \$15 on the bagels. She had \$23 in beginning, so now she has \$23 - \$15 = \$8. The answer is 8. \\
        \bottomrule
    \end{tabular}
\end{table}
\endgroup

==> demonstrations/Normal-CoT-Commonsense-CSQA.tex <==
\begingroup
\begin{table}[htb]
    \centering
    \caption{
    Normal CoT - Commonsense CSQA. 
    }
    \vspace{2.8mm}
    \begin{tabular}{p{0.96\linewidth}}
        \toprule
        \textbf{Q:} What do people use to absorb extra ink from a fountain pen? Answer Choices: (a) shirt pocket (b) calligrapher’s hand (c) inkwell (d) desk drawer (e) blotter \\
\vspace{-1mm}
\textbf{A:} The answer must be an item that can absorb ink. Of the above choices, only blotters are used to absorb ink. So the answer is (e). \\
\vspace{0mm}
\textbf{Q:} What home entertainment equipment requires cable? Answer Choices: (a) radio shack (b) substation (c) television (d) cabinet \\
\vspace{-1mm}
\textbf{A:} The answer must require cable. Of the above choices, only television requires cable. So the answer is (c). \\
\vspace{0mm}
\textbf{Q:} The fox walked from the city into the forest, what was it looking for? Answer Choices: (a) pretty flowers (b) hen house (c) natural habitat (d) storybook \\
\vspace{-1mm}
\textbf{A:} The answer must be something in the forest. Of the above choices, only natural habitat is in the forest. So the answer is (b). \\
\vspace{0mm}
\textbf{Q:} Sammy wanted to go to where the people were. Where might he go? Answer Choices: (a) populated areas (b) race track (c) desert (d) apartment (e) roadblock \\
\vspace{-1mm}
\textbf{A:} The answer must be a place with a lot of people. Of the above choices, only populated areas have a lot of people. So the answer is (a). \\
\vspace{0mm}
\textbf{Q:} Where do you put your grapes just before checking out? Answer Choices: (a) mouth (b) grocery cart (c) super market (d) fruit basket (e) fruit market \\
\vspace{-1mm}
\textbf{A:} The answer should be the place where grocery items are placed before checking out. Of the above choices, grocery cart makes the most sense for holding grocery items. So the answer is (b). \\
\vspace{0mm}
\textbf{Q:} Google Maps and other highway and street GPS services have replaced what? Answer Choices: (a) united states (b) mexico (c) countryside (d) atlas \\
\vspace{-1mm}
\textbf{A:} The answer must be something that used to do what Google Maps and GPS services do, which is to give directions. Of the above choices, only atlases are used to give directions. So the answer is (d). \\
\vspace{0mm}
\textbf{Q:} Before getting a divorce, what did the wife feel who was doing all the work? Answer Choices: (a) harder (b) anguish (c) bitterness (d) tears (e) sadness \\
\vspace{-1mm}
\textbf{A:} The answer should be the feeling of someone getting divorced who was doing all the work. Of the above choices, the closest feeling is bitterness. So the answer is (c). \\
\bottomrule
    \end{tabular}
\end{table}
\endgroup

==> demonstrations/Normal-CoT-Commonsense-Date.tex <==
\begingroup
\begin{table}[htb]
    \centering
    \caption{
    Normal CoT - Commonsense - Date. 
    }
    \vspace{2.8mm}
    \begin{tabular}{p{0.96\linewidth}}
        \toprule
        \textbf{Q:} There are 15 trees in the grove. Grove workers will plant trees in the grove today. After they are done, there will be 21 trees. How many trees did the grove workers plant today? \\
\vspace{-1mm}
\textbf{A:} We start with 15 trees. Later we have 21 trees. The difference must be the number of trees they planted. So, they must have planted 21 - 15 = 6 trees. The answer is 6. \\
\vspace{0mm}
\textbf{Q:} If there are 3 cars in the parking lot and 2 more cars arrive, how many cars are in the parking lot? \\
\vspace{-1mm}
\textbf{A:} There are 3 cars in the parking lot already. 2 more arrive. Now there are 3 + 2 = 5 cars. The answer is 5. \\
\vspace{0mm}
\textbf{Q:}  Leah had 32 chocolates and her sister had 42. If they ate 35, how many pieces do they have left in total? \\
\vspace{-1mm}
\textbf{A:} Leah had 32 chocolates and Leah’s sister had 42. That means there were originally 32 + 42 = 74 chocolates. 35 have been eaten. So in total they still have 74 - 35 = 39 chocolates. The answer is 39. \\
\vspace{0mm}
\textbf{Q:} Jason had 20 lollipops. He gave Denny some lollipops. Now Jason has 12 lollipops. How many lollipops did Jason give to Denny? \\
\vspace{-1mm}
\textbf{A:} Jason had 20 lollipops. Since he only has 12 now, he must have given the rest to Denny. The number of lollipops he has given to Denny must have been 20 - 12 = 8 lollipops. The answer is 8. \\
\vspace{0mm}
\textbf{Q:} Shawn has five toys. For Christmas, he got two toys each from his mom and dad. How many toys does he have now? \\
\vspace{-1mm}
\textbf{A:} He has 5 toys. He got 2 from mom, so after that he has 5 + 2 = 7 toys. Then he got 2 more from dad, so in total he has 7 + 2 = 9 toys. The answer is 9.  \\
\vspace{0mm}
\textbf{Q:} There were nine computers in the server room. Five more computers were installed each day, from monday to thursday. How many computers are now in the server room? \\
\vspace{-1mm}
\textbf{A:} There are 4 days from monday to thursday. 5 computers were added each day. That means in total 4 * 5 = 20 computers were added. There were 9 computers in the beginning, so now there are 9 + 20 = 29 computers. The answer is 29. \\
\vspace{0mm}
\textbf{Q:} Michael had 58 golf balls. On tuesday, he lost 23 golf balls. On wednesday, he lost 2 more. How many golf balls did he have at the end of wednesday? \\
\vspace{-1mm}
\textbf{A:} Michael initially had 58 balls. He lost 23 on Tuesday, so after that he has 58 - 23 = 35 balls. On Wednesday he lost 2 more so now he has 35 - 2 = 33 balls. The answer is 33. \\
\vspace{0mm}Michael initially had 58 balls. He lost 23 on Tuesday, so after that he has 58 - 23 = 35 balls. On Wednesday he lost 2 more so now he has 35 - 2 = 33 balls. The answer is 33.
\textbf{Q:} Olivia has \$23. She bought five bagels for \$3 each. How much money does she have left? \\
\vspace{-1mm}
\textbf{A:}  She bought 5 bagels for \$3 each. This means she spent 5 * \$3 = \$15 on the bagels. She had \$23 in beginning, so now she has \$23 - \$15 = \$8. The answer is 8. \\
\bottomrule
    \end{tabular}
\end{table}
\endgroup
